RigGS: Rigging of 3D Gaussians for Modeling Articulated Objects in Videos

This paper considers the problem of modeling articulated objects captured in 2D videos to enable novel view synthesis, while also being easily editable, drivable, and re-posable. To tackle this challenging problem, we propose RigGS, a new paradigm that leverages 3D Gaussian representation and skeleton-based motion representation to model dynamic objects without utilizing additional template priors. Specifically, we first propose skeleton-aware node-controlled deformation, which deforms a canonical 3D Gaussian representation over time to initialize the modeling process, producing candidate skeleton nodes that are further simplified into a sparse 3D skeleton according to their motion and semantic information. Subsequently, based on the resulting skeleton, we design learnable skin deformations and pose-dependent detailed deformations, thereby easily deforming the 3D Gaussian representation to generate new actions and render further high-quality images from novel views. Extensive experiments demonstrate that our method can generate realistic new actions easily for objects and achieve high-quality rendering.

==> table_scripts/running_time.tex <==
\begin{table}[h]
	\caption{Comparisons of the running time.}
	\label{Tab:time}
		\setlength{\tabcolsep}{3pt}
	\centering
	\begin{small}
		\begin{tabular}{ c | c c c c c c}
            \toprule 
            Method & D-NeRF~\cite{pumarola2021dnerf} & TiNeuVox~\cite{fang2022TiNeuVox} & 4D-GS~\cite{wu20244dgs} & SC-GS~\cite{huang2024sc} & AP-NeRF~\cite{uzolas2024template} & Ours\\
            Training & 20 h & & & 40min & & 3h 10min \\
            Inference & & & & 0.005s & & 0.03s\\
            \bottomrule
		\end{tabular}
	\end{small}
\end{table}

